Learning Explicit Object-Centric Representations with Vision Transformers

With the recent successful adaptation of transformers to the vision domain, particularly when trained in a self-supervised fashion, it has been shown that vision transformers can learn impressive object-reasoning-like behaviour and features expressive for the task of object segmentation in images. In this paper, we build on the self-supervision task of masked autoencoding and explore its effectiveness for explicitly learning object-centric representations with transformers. To this end, we design an object-centric autoencoder using transformers only and train it end-to-end to reconstruct full images from unmasked patches. We show that the model efficiently learns to decompose simple scenes as measured by segmentation metrics on several multi-object benchmarks.

==> architecture/architecture.tex <==
%% Architecture drawing specifics

\tikzstyle{text} = [font=\large, text centered]

\tikzstyle{cls} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black]

\tikzstyle{patch} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black, fill=cyan!30]

\tikzstyle{masked_patch} = [rectangle, rounded corners, minimum width=0.5cm, minimum height=0.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{dot_product} = [circle, rounded corners, minimum width=0.2cm, minimum height=0.2cm,text centered, draw=black, scale=0.6]

\tikzstyle{encoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=6.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{function} = [rectangle, rounded corners,text centered, align=center, draw=black]

\tikzstyle{decoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=2cm,text centered, draw=black, fill=gray!30]


\begin{tikzpicture}[]

\node (input) at (-1,0) [] {\includegraphics[width=60pt]{architecture/images/input.png}};

\node (unmasked) at (-1,4.75) [] {\includegraphics[height=110pt]{architecture/images/unmasked.png}};

\node (cls_0) at (1,9) [cls, fill=red!30] {};
\node (cls_1) at (1,8.5) [cls, fill=blue!30] {};
\node (cls_2) at (1,8) [cls, fill=green!30] {};
\node (cls_3) at (1,7.5) [cls, fill=yellow!30] {};

\node (patch_0) at (1,6.5) [patch] {};
\node (patch_1) at (1,6) [patch] {};
\node (patch_2) at (1,5.5) [patch] {};
\node (patch_3) at (1,5) [patch] {};
\node (patch_4) at (1,4.5) [patch] {};
\node (patch_5) at (1,4) [patch] {};
\node (patch_6) at (1,3.5) [patch] {};
\node (patch_7) at (1,3) [patch] {};

\node (encoder) at (3,6) [encoder] {Encoder};

\node (cls_0_enc) at (5,9) [cls, fill=red!30] {};
\node (cls_1_enc) at (5,8.5) [cls, fill=blue!30] {};
\node (cls_2_enc) at (5,8) [cls, fill=green!30] {};
\node (cls_3_enc) at (5,7.5) [cls, fill=yellow!30] {};

\node (patch_0_enc) at (5,6.5) [patch] {};
\node (patch_1_enc) at (5,6) [patch] {};
\node (patch_2_enc) at (5,5.5) [patch] {};
\node (patch_3_enc) at (5,5) [patch] {};
\node (patch_4_enc) at (5,4.5) [patch] {};
\node (patch_5_enc) at (5,4) [patch] {};
\node (patch_6_enc) at (5,3.5) [patch] {};
\node (patch_7_enc) at (5,3) [patch] {};

\node (extraction) at (7,4.75) [function, minimum height=2cm, fill=gray!30] {Object \\ function};

\node (text) at (9,5.5) [] {$\mathbf{a}$};
\node (text) at (9,4) [] {$\mathbf{s}$};

\node (forming) at (11,4.75) [function, minimum height=2cm, fill=gray!30] {Position \\ function};


\foreach \Z/\C in {-1.5/yellow,-1/green,-0.5/blue, 0/red}
{
\node (patch_0_mask) at (13,6.5,\Z) [cls, fill=\C!30] {};
\node (patch_1_mask) at (13,6,\Z) [cls, fill=\C!30] {};
\node (patch_2_mask) at (13,5.5,\Z) [cls, fill=gray!30] {};
\node (dots) at (13,4.9,\Z) [] {$\vdots$};
\node (patch_5_mask) at (13,4,\Z) [cls, fill=gray!30] {};
\node (patch_6_mask) at (13,3.5,\Z) [cls, fill=gray!30] {};
\node (patch_7_mask) at (13,3,\Z) [cls, fill=\C!30] {};
}

\foreach \Z in {-1.5,-1,-0.5, 0}
{
\node (decoder) at (15.5,4.75, \Z) [decoder] {Decoder};
}

\foreach \Z/\C in {-1.5/yellow,-1/green,-0.5/blue, 0/red}
{
\node (patch_0_mask) at (18,6.5,\Z) [cls, fill=\C!30] {};
\node (patch_1_mask) at (18,6,\Z) [cls, fill=\C!30] {};
\node (patch_2_mask) at (18,5.5,\Z) [cls, fill=\C!30] {};
\node (dots) at (18,4.9,\Z) [] {$\vdots$};
\node (patch_5_mask) at (18,4,\Z) [cls, fill=\C!30] {};
\node (patch_6_mask) at (18,3.5,\Z) [cls, fill=\C!30] {};
\node (patch_7_mask) at (18,3,\Z) [cls, fill=\C!30] {};
}

\node (out_patch_first) at (20.5,6) [] {\includegraphics[height=41.25pt]{architecture/images/first3.png}};
\node (dots) at (20.5,4.9) [] {$\vdots$};
\node (out_patch_first) at (20.5,3.5) [] {\includegraphics[height=41.25pt]{architecture/images/last3.png}};

\node (output) at (20.5,0) [] {\includegraphics[width=60pt]{architecture/images/output.png}};

\draw [-to, thick](-1,1.25) -- (-1,2.25);
\draw [-to, thick](-0.5,4.75) -- (0.5,4.75);
\draw [-to, thick](1.5,4.75) -- (1.75,4.75);
\draw [-to, thick](4.25,4.75) -- (4.5,4.75);
\draw [-to, thick](1.5,8.25) -- (1.75,8.25);
\draw [-to, thick](4.25,8.25) -- (4.5,8.25);
\draw [-to, thick](5.5,8.25) -| (7,6);
\draw [-to, thick](5.5,4.75) -- (5.75,4.75);
\draw [-to, thick](8.25,5.5) -- (8.5,5.5);
\draw [-to, thick](8.25,4) -- (8.5,4);
\draw [-to, thick](9.5,5.5) -- (9.75,5.5);
\draw [-to, thick](9.5,4) -- (9.75,4);
\draw [-to, thick](12.25,4.75) -- (12.5,4.75);
\draw [-to, thick](14,4.75) -- (14.25,4.75);
\draw [-to, thick](17.25,4.75) -- (17.5,4.75);
\draw [-to, thick](19,4.75) -- (20,4.75);
\draw [-to, thick](20.5,2.25) -- (20.5,1.25);

\end{tikzpicture}

==> architecture/object_function.tex <==

\tikzstyle{text} = [font=\large, text centered]

\tikzstyle{cls} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black]

\tikzstyle{patch} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black, fill=cyan!30]

\tikzstyle{masked_patch} = [rectangle, rounded corners, minimum width=0.5cm, minimum height=0.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{dot_product} = [circle, rounded corners, minimum width=0.2cm, minimum height=0.2cm,text centered, draw=black, scale=0.6]

\tikzstyle{encoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=6.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{function} = [rectangle, rounded corners,text centered, align=center, draw=black]

\tikzstyle{decoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=2cm,text centered, draw=black, fill=gray!30]

\begin{tikzpicture}[]
  
    \node (cls_0_enc) at (0,6) [cls, fill=red!30] {};
    \node (cls_1_enc) at (0,5.5) [cls, fill=blue!30] {};
    \node (cls_2_enc) at (0,5) [cls, fill=green!30] {};
    \node (cls_3_enc) at (0,4.5) [cls, fill=yellow!30] {};
  
    \node (patch_0_enc) at (0,3.5) [patch] {};
    \node (patch_1_enc) at (0,3) [patch] {};
    \node (patch_2_enc) at (0,2.5) [patch] {};
    \node (patch_3_enc) at (0,2) [patch] {};
    \node (patch_4_enc) at (0,1.5) [patch] {};
    \node (patch_5_enc) at (0,1) [patch] {};
    \node (patch_6_enc) at (0,0.5) [patch] {};
    \node (patch_7_enc) at (0,0) [patch] {};
    
    \node (dot_product) at (3,1.75) [function, fill=gray!30] {Scaled\\dot\\product};
    
    \node (softmax) at (6,1.75) [function, fill=purple!30] {Softmax};
    
    \node (w_mean) at (9,1.75) [function, fill=gray!30] {Weighted\\mean};
    
    \node (text) at (12,3.5) [] {$\mathbf{a}$};
    \node (text) at (12,1.75) [] {$\mathbf{s}$};

    \draw [-to, thick](0.5,5.25) -| (3,3);
    \draw [-to, thick](0.5,1.75) -- (1.75,1.75);
    \draw [-to, thick](4,1.75) -- (4.75,1.75);
    \draw [-to, thick](7,1.75) -- (7.75,1.75);
    \draw [-to, thick](7.375,1.75) |- (11.5,3.5);
    \draw [-to, thick](10.25,1.75) -- (11.5,1.75);
    \draw [-to, thick](1.125,1.75) |- (6,0) -| (9,1);
\end{tikzpicture}
   

==> architecture/position_function.tex <==
\tikzstyle{text} = [font=\large, text centered]

\tikzstyle{cls} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black]

\tikzstyle{patch} = [rectangle, rounded corners, minimum width=0.4cm, minimum height=0.4cm,text centered, draw=black, fill=cyan!30]

\tikzstyle{masked_patch} = [rectangle, rounded corners, minimum width=0.5cm, minimum height=0.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{dot_product} = [circle, rounded corners, minimum width=0.2cm, minimum height=0.2cm,text centered, draw=black, scale=0.6]

\tikzstyle{encoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=6.5cm,text centered, draw=black, fill=gray!30]

\tikzstyle{function} = [rectangle, rounded corners,text centered, align=center, draw=black]

\tikzstyle{decoder} = [rectangle, rounded corners, minimum width=1cm, minimum height=2cm,text centered, draw=black, fill=gray!30]

\begin{tikzpicture}[]
  
    \node (text) at (0,3.5) [] {$\log\mathbf{a}$};
    \node (text) at (0,0) [] {$\mathbf{s}$};
    

     \node (broadcast) at (3,0) [function, fill=gray!30] {Broadcast};
    
    \node (concatenate) at (3,1.75) [function, fill=gray!30] {Concatenate};
    
    \node (project) at (7.25,1.75) [function, fill=gray!30] {Project};
    
    
    \node (add) at (11,1.75) [function, fill=gray!30] {Add\\ mask\\tokens};
    
    \node (unshuffle) at (14.5,1.75) [function, fill=gray!30] {Unshuffle};
    
    \foreach \Z/\C in {-1.5/yellow,-1/green,-0.5/blue, 0/red}
    {
    \node (patch_0_mask) at (17.5,3.5,\Z) [cls, fill=\C!30] {};
    \node (patch_1_mask) at (17.5,3,\Z) [cls, fill=\C!30] {};
    \node (patch_2_mask) at (17.5,2.5,\Z) [cls, fill=gray!30] {};
    \node (dots) at (17.5,1.9,\Z) [] {$\vdots$};
    \node (patch_5_mask) at (17.5,1,\Z) [cls, fill=gray!30] {};
    \node (patch_6_mask) at (17.5,0.5,\Z) [cls, fill=gray!30] {};
    \node (patch_7_mask) at (17.5,0,\Z) [cls, fill=\C!30] {};
    }
    
    \draw [-to, thick](0.75,3.5) -| (3,2.25);
    \draw [-to, thick](0.75,0) -- (1.75,0);
    \draw [-to, thick](3,0.5) -- (3,1.25);
    \draw [-to, thick](4.5,1.75) -- (6.25,1.75);
    \draw [-to, thick](8.25,1.75) -- (10,1.75);
    \draw [-to, thick](12,1.75) -- (13.25,1.75);
    \draw [-to, thick](15.75,1.75) -- (17,1.75);
\end{tikzpicture}

